The new $(g-2)_\mu$ result and the $\mu\nu$SSM

The $\mu\nu$SSM is a highly predictive alternative model to the MSSM. In particular, the electroweak sector of the model can explain the longstanding discrepancy between the experimental result for the anomalous magnetic moment of the muon, $(g-2)_\mu$, and its Standard Model prediction, while being in agreement with all other theoretical and experimental constraints. The recently published MUON G-2 result is within $0.8\,\sigma$ in agreement with the older BNL result on $(g-2)_\mu$. The combined result was announced as $a_\mu^{\rm exp} = (11659206.1 \pm 4.1) \times 10^{-10}$, yielding a new deviation from the Standard Model prediction of $\Delta a_\mu = (25.1 \pm 5.9) \times 10^{-10}$, corresponding to $4.2\,\sigma$. Using this improved bound we update the analysis in the $\mu\nu$SSM as presented in Ref. [1] and set new limits on the allowed parameters space of the electroweak sector of the model. We conclude that significant regions of the model can explain the new $(g-2)_\mu$ data.

==> paperdef.tex <==

\newcommand{\lsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle <}{\sim}$}\;}
\newcommand{\gsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle >}{\sim}$}\;}

\newcommand\Code[1]{\ensuremath{\texttt{#1}}}
\newcommand\Var[1]{\ensuremath{\mathit{#1}}}
\newcommand\Vi{\Var{i}}
\newcommand\Vj{\Var{j}}
\newcommand\Vt{\Var{t}}
\newcommand\Vg{\Var{g}}
\newcommand\Vs{\Var{s}}

\newcommand\al{\alpha}
\newcommand\be{\beta}
\newcommand\tb{\tan\beta}
\newcommand\TB{t_\beta}
\newcommand\SB{s_\beta}
\newcommand\CB{c_\beta}
\newcommand\CBB{c_{2\beta}}
\newcommand\SA{s_\alpha}
\newcommand\CA{c_\alpha}
\newcommand\CBA{c_{\beta - \alpha}}
\newcommand\SBA{s_{\beta - \alpha}}
\newcommand\CAB{c_{\alpha + \beta}}
\newcommand\SAB{s_{\alpha + \beta}}

\newcommand\LP{\left(}
\newcommand\RP{\right)}
\newcommand\LB{\left[}
\newcommand\RB{\right]}
\newcommand\LV{\left\{}
\newcommand\RV{\right\}}
\newcommand\ra{\rightarrow}
\newcommand\tenp[1]{\times 10^{#1}}

\renewcommand\Re{\mathop{\mathrm{Re}}}
\renewcommand\Im{\mathop{\mathrm{Im}}}
\newcommand\ReTilde{\mathop{\widetilde{\mathrm{Re}}}}
\newcommand\ReDiag{\mathop{%
  \raise .5pt\hbox{[}%
  \widetilde{\mathrm{Re}}%
  \raise .5pt\hbox{]}}}
\newcommand\ReOffDiag{\mathop{%
  \raise .5pt\hbox{$\llbracket$}%
  \widetilde{\mathrm{Re}}%
  \raise .5pt\hbox{$\rrbracket$}}}
\newcommand\SE[1]{\Sigma_{#1}}
\newcommand\OS{\mathrm{OS}}
\newcommand\DRbar{\ensuremath{\smash{\overline{\mathrm{DR}}}}}
\newcommand\MSbar{\ensuremath{\overline{\mathrm{MS}}}}
\newcommand\matr[1]{\mathbf{#1}}
\newcommand\mati[1]{\bigl(#1\bigr)}
\newcommand\unity{\mathrm{1\mskip-4.25mu l}}
\newcommand\ddiv{\bigr|_{\mathrm{div}}}
\newcommand\Ddiv{\Bigr|_{\mathrm{div}}}
\newcommand\cMt{{\cal M}_{\text{tree}}}
\newcommand\cMl{{\cal M}_{\text{1-loop}}}
\newcommand\cL{{\cal L}}

\newcommand\SW{s_\mathrm{w}}
\newcommand\CW{c_\mathrm{w}}
\newcommand\MW{M_W}
\newcommand\MZ{M_Z}
\newcommand\Mh{M_h}
\newcommand\MH{M_H}
\newcommand\MA{M_A}
\newcommand\MHp{M_{H^\pm}}
\newcommand\mf[1]{m_{f_{#1}}}
\newcommand\mb{m_b}
\newcommand\mt{m_t}
\newcommand\Ab{A_b}
\newcommand\At{A_t}
\newcommand\Atau{A_\tau}
\newcommand\Amu{A_\mu}
\newcommand\Ae{A_e}

\newcommand\Sf{\tilde f}
\newcommand\Sfp{\tilde f^\prime}
\newcommand\msf[1]{m_{\Sf_{#1}}}
\newcommand\msfp[1]{m_{\Sfp_{#1}}}
\newcommand\Sn{\tilde\nu}
\newcommand\Sl{\tilde l}
\newcommand\sle[1]{\tilde l_{#1}}
\newcommand\Slpm{\tilde l^\pm}
\newcommand\msn[1]{m_{\Sn_{#1}}}
\newcommand\Sel[1]{\tilde e_{#1}}
\newcommand\Smu[1]{\tilde \mu_{#1}}
\newcommand\Fe{\mathrm{e}}
\newcommand\mfe[1]{m_{\Fe_{#1}}}
\newcommand\mse[1]{m_{\Sel{#1}}}
\newcommand\msl[1]{m_{\Sl_{#1}}}
\newcommand\Su{\mathrm{\tilde u}}
\newcommand\Fu{\mathrm{u}}
\newcommand\mfu[1]{m_{\Fu_{#1}}}
\newcommand\msu[1]{m_{\Su_{#1}}}
\newcommand\Sd{\mathrm{\tilde d}}
\newcommand\Fd{\mathrm{d}}
\newcommand\mfd[1]{m_{\Fd_{#1}}}
\newcommand\msd[1]{m_{\Sd_{#1}}}
\newcommand\hmsu[1]{\hat m_{\Su_{#1}}}
\newcommand\hmsd[1]{\hat m_{\Sd_{#1}}}
\newcommand\Stau[1]{{\tilde\tau_{#1}}}
\newcommand\stau{\tilde \tau}
\newcommand\Stop[1]{{\tilde t_{#1}}}
\renewcommand\stop{\tilde t}
\newcommand\Sbot[1]{{\tilde b_{#1}}}
\newcommand\sbot{\tilde b}

\newcommand\mL{m_{\tilde l_L}}
\newcommand\mR{m_{\tilde l_R}}
\newcommand\msnu{m_{\tilde \nu_l}}

\newcommand\cind{c^{\phantom{\prime}}}
\newcommand\cpri{c^\prime}
\newcommand\nind{n^{\phantom{\prime}}}
\newcommand\npri{n^\prime}
\newcommand\sind{s^{\phantom{\prime}}}
\newcommand\spri{s^{\prime}}
\newcommand\dZ[1]{\delta Z_{#1}}
\newcommand\dZm[1]{\delta\matr{Z}_{#1}}
\newcommand\dbZm[1]{\delta\matr{\breve Z}_{#1}}
\newcommand\dBZm[1]{\delta\matr{\breve{\bar Z}}{}_{#1}}

\newcommand\gl{{\tilde g}}
\newcommand\mgl{m_\gl}
\newcommand\phigl{\varphi_\gl}
\newcommand\dTB{\delta\TB}
\newcommand\ino[1]{\tilde\chi_{#1}}
\newcommand\mino[1]{m_{\ino{#1}}}
\newcommand\chapm[1]{\ino{#1}^\pm}
\newcommand\champ[1]{\ino{#1}^\mp}
\newcommand\chap[1]{\ino{#1}^+}
\newcommand\cham[1]{\ino{#1}^-}
\newcommand\cha{\chapm}
\newcommand\mcha[1]{m_{\chapm{#1}}}
\newcommand\mchap[1]{m_{\ino{#1}^+}}
\newcommand\mcham[1]{m_{\ino{#1}^-}}
\newcommand\neu[1]{\ino{#1}^0}
\newcommand\mneu[1]{m_{\neu{#1}}}

\newcommand\refeq[1]{Eq.~(\ref{#1})}
\newcommand\refeqs[1]{Eqs.~(\ref{#1})}
\newcommand\refta[1]{Tab.~\ref{#1}}
\newcommand\refse[1]{Sect.~\ref{#1}}
\newcommand\refses[1]{Sects.~\ref{#1}}
\newcommand\citere[1]{Ref.~\cite{#1}}
\newcommand\citeres[1]{Refs.~\cite{#1}}

\newcommand\lbrac{\symbol{123}}
\newcommand\rbrac{\symbol{125}}
\newcommand\Brac[1]{\lbrac#1\rbrac}
\newcommand\uscore{\symbol{95}}
\newcommand\eg{e.g.}
\newcommand\ie{i.e.\ }
\newcommand\wrt{w.r.t.\ }

\newcommand{\SM}{\mathrm{SM}}
\newcommand{\MSSM}{\mathrm{MSSM}}
\newcommand{\NMSSM}{\mathrm{NMSSM}}
\newcommand{\mnSSM}{\ensuremath{\mu\nu\mathrm{SSM}}}

\newcommand\trans{T}
\newcommand{\CP}{{\cal CP}}
\newcommand{\cp}{{\CP}}
\newcommand{\os}{\mathrm{os}}
\newcommand{\wtre}{\widetilde\Re}
\newcommand{\wtim}{\widetilde\Im}
\newcommand{\onel}{one-loop}
\newcommand{\tev}{\,\, \mathrm{TeV}}
\newcommand{\gev}{\,\, \mathrm{GeV}}
\newcommand{\mev}{\,\, \mathrm{MeV}}
\newcommand{\kev}{\,\, \mathrm{keV}}
\newcommand{\Hpm}{H^\pm}
\newcommand{\He}{h_1}
\newcommand{\Hz}{h_2}
\newcommand{\Hd}{h_3}

\newcommand{\eehh}{e^+e^- \to h_i h_j}
\newcommand{\eehZ}{e^+e^- \to h_i Z}
\newcommand{\eehga}{e^+e^- \to h_i \ga}

\newcommand{\eeHH}{e^+e^- \to H^+ H^-}
\newcommand{\eeHW}{e^+e^- \to H^{\pm} W^{\mp}}
\newcommand{\eeHpWm}{e^+e^- \to H^{+} W^{-}}
\newcommand{\eeHmWp}{e^+e^- \to H^{-} W^{+}}

\newcommand{\eecc}{\ensuremath{e^+e^- \to \chapm{c} \champ{\cpri}}}
\newcommand{\eecece}{e^+e^- \to \chap1 \cham1}
\newcommand{\eececz}{e^+e^- \to \chapm1 \champ2}
\newcommand{\eeczcz}{e^+e^- \to \chap2 \cham2}
\newcommand{\eecmcp}{e^+e^- \to \cham{c} \chap{\cpri}}
\newcommand{\eecpcm}{e^+e^- \to \chap{c} \cham{\cpri}}
\newcommand{\eecepczm}{e^+e^- \to \chap1 \cham2}
\newcommand{\eecemczp}{e^+e^- \to \cham1 \chap2}
\newcommand{\eeczpcem}{e^+e^- \to \chap2 \cham1}

\newcommand{\eenn}{\ensuremath{e^+e^- \to \neu{n} \neu{\npri}}}
\newcommand{\eenene}{e^+e^- \to \neu1 \neu1}
\newcommand{\eenznz}{e^+e^- \to \neu2 \neu2}
\newcommand{\eendnd}{e^+e^- \to \neu3 \neu3}
\newcommand{\eenvnv}{e^+e^- \to \neu4 \neu4}
\newcommand{\eenenz}{e^+e^- \to \neu1 \neu2}
\newcommand{\eenend}{e^+e^- \to \neu1 \neu3}
\newcommand{\eenenv}{e^+e^- \to \neu1 \neu4}
\newcommand{\eenznd}{e^+e^- \to \neu2 \neu3}
\newcommand{\eenznv}{e^+e^- \to \neu2 \neu4}
\newcommand{\eendnv}{e^+e^- \to \neu3 \neu4}

\newcommand{\eeSlSl}{\ensuremath{e^+e^- \to \Sl_{gs} \Sl_{gs^{\prime}}}}
\newcommand{\eeSeSe}{\ensuremath{e^+e^- \to \Se^{\pm}_{gs} \Se^{\mp}_{gs^{\prime}}}}
\newcommand{\eeSeeSee}{\ensuremath{e^+e^- \to \tilde{e}^+_1 \tilde{e}^-_1}}
\newcommand{\eeSeeSez}{\ensuremath{e^+e^- \to \tilde{e}^{\pm}_1 \tilde{e}^{\mp}_2}}
\newcommand{\eeSezSez}{\ensuremath{e^+e^- \to \tilde{e}^+_2 \tilde{e}^-_2}}
\newcommand{\eeSmeSme}{\ensuremath{e^+e^- \to \tilde{\mu}^+_1 \tilde{\mu}^-_1}}
\newcommand{\eeSmeSmz}{\ensuremath{e^+e^- \to \tilde{\mu}^{\pm}_1 \tilde{\mu}^{\mp}_2}}
\newcommand{\eeSmzSmz}{\ensuremath{e^+e^- \to \tilde{\mu}^+_2 \tilde{\mu}^-_2}}
\newcommand{\eeSaeSae}{\ensuremath{e^+e^- \to \tilde{\tau}^+_1 \tilde{\tau}^-_1}}
\newcommand{\eeSaeSaz}{\ensuremath{e^+e^- \to \tilde{\tau}^{\pm}_1 \tilde{\tau}^{\mp}_2}}
\newcommand{\eeSazSaz}{\ensuremath{e^+e^- \to \tilde{\tau}^+_2 \tilde{\tau}^-_2}}
\newcommand{\eeSnSn}{\ensuremath{e^+e^- \to \Sn_{g} \Sn_{g}}}
\newcommand{\eeSneSne}{\ensuremath{e^+e^- \to \tilde{\nu}_e \tilde{\nu}_e}}
\newcommand{\eeSnmSnm}{\ensuremath{e^+e^- \to \tilde{\nu}_{\mu} \tilde{\nu}_{\mu}}}
\newcommand{\eeSnaSna}{\ensuremath{e^+e^- \to \tilde{\nu}_{\tau} \tilde{\nu}_{\tau}}}

\newcommand\hChaDecay{h_i \to \cham{c} \chap{\cpri}}
\newcommand\hchaechae{h_i \to \champ1 \chapm1}
\newcommand\hchaechaz{h_i \to \champ1 \chapm2}
\newcommand\hchazchaz{h_i \to \champ2 \chapm2}
\newcommand\hNeuDecay{h_i \to \neu{n} \neu{\npri}}
\newcommand\hneueneue{h_i \to \neu1 \neu1}
\newcommand\hneuzneuz{h_i \to \neu2 \neu2}
\newcommand\hneudneud{h_i \to \neu3 \neu3}
\newcommand\hneuvneuv{h_i \to \neu4 \neu4}
\newcommand\hneueneuz{h_i \to \neu1 \neu2}
\newcommand\hneueneud{h_i \to \neu1 \neu3}
\newcommand\hneueneuv{h_i \to \neu1 \neu4}
\newcommand\hneuzneud{h_i \to \neu2 \neu3}
\newcommand\hneuzneuv{h_i \to \neu2 \neu4}
\newcommand\hneudneuv{h_i \to \neu3 \neu4}

\newcommand\hzstst{h_2 \to \Stop1 \Stop2, \Stop2 \Stop1}
\newcommand\hdstst{h_3 \to \Stop1 \Stop2, \Stop2 \Stop1}
\newcommand\hnstst{h_n \to \Stop1 \Stop2, \Stop2 \Stop1}
\newcommand\hzsbsb{h_2 \to \Sbot1 \Sbot2, \Sbot2 \Sbot1}
\newcommand\hnsbsb{h_n \to \Sbot1 \Sbot2, \Sbot2 \Sbot1}
\newcommand\hnstaustau{h_n \to \Stau1 \Stau2, \Stau2 \Stau1}
\newcommand\Hpdecay{H^+ \to \neu{n} \chap{c}}
\newcommand\Hmdecay{H^- \to \neu{n} \cham{c}}
\newcommand\HpmDecay{H^\pm \to \neu{n} \chapm{c}}
\newcommand\decayxy{H \to \text{xy}}
\newcommand\edz{\tfrac{1}{2}}
\newcommand\FA{\texttt{FeynArts}}
\newcommand\FC{\texttt{FormCalc}}
\newcommand\LT{\texttt{LoopTools}}
\newcommand\FH{\texttt{FeynHiggs}}
\newcommand\fh{\texttt{FeynHiggs}}
\newcommand\FT{\texttt{FeynTools}}
\newcommand\MO{\texttt{MicrOMEGAs}}
\newcommand\CM{\texttt{CheckMATE}}
\newcommand\HDECAY{\texttt{HDECAY}}
\newcommand\Sq{{\tilde q}}
\newcommand\msq[1]{m_{\Sq_{#1}}}
\newcommand\Mt{\tilde{M}}
\newcommand\pb{\ensuremath{\mbox{pb}}}
\newcommand\fb{\ensuremath{\mbox{fb}}}
\newcommand\ab{\ensuremath{\mbox{ab}}}
\newcommand\ipb{\ensuremath{\pb^{-1}}}
\newcommand\ifb{\ensuremath{\fb^{-1}}}
\newcommand\iab{\ensuremath{\ab^{-1}}}

\newcommand\mh[1]{m_{h_{#1}}}
\newcommand\msqua[1]{m_{\tilde{q}_{#1}}}
\newcommand\mstop[1]{m_{\tilde{t}_{#1}}}
\newcommand\msbot[1]{m_{\tilde{b}_{#1}}}
\newcommand\msele[1]{m_{\tilde{e}_{#1}}}
\newcommand\msmu[1]{m_{\tilde{\mu}_{#1}}}
\newcommand\mstau[1]{m_{\tilde{\tau}_{#1}}}
\newcommand\msneu{m_{\tilde{\nu}_{e,\mu,\tau}}}
\newcommand\melesneu{m_{\tilde{\nu}_{e}}}
\newcommand\mmuesneu{m_{\tilde{\nu}_{\mu}}}
\newcommand\mtausneu{m_{\tilde{\nu}_{\tau}}}

\newcommand{\Scs}{$\mathcal S$}
\newcommand{\Sce}{S1}
\newcommand{\Scz}{S2}
\newcommand{\Scd}{S3}
\newcommand{\Scv}{S4}
\newcommand{\Scf}{S5}
\newcommand{\br}{\text{BR}}
\newcommand{\db}{\Delta_b}
\newcommand{\rmd}{\text{d}}

\newcommand{\sig}{\sigma}
\newcommand{\sigfull}{\sigma_{\text{full}}}
\newcommand{\sigtree}{\sigma_{\text{tree}}}
\newcommand{\sigloop}{\sigma_{\text{loop}}}
\newcommand{\sigweak}{\sigma_{\text{weak}}}
\newcommand{\sigvirt}{\sigma_{\text{virt}}}
\newcommand{\sigsoft}{\sigma_{\text{soft}}}
\newcommand{\sighard}{\sigma_{\text{hard}}}
\newcommand{\sigcoll}{\sigma_{\text{coll}}}

\newcommand{\StopL}{\tilde{t}_L}
\newcommand{\StopR}{\tilde{t}_R}
\newcommand{\Snutau}{\tilde{\nu}_\tau}

\newcommand{\phiAeg}{\varphi_{A_{\Fe_g}}}
\newcommand{\phiAug}{\varphi_{A_{\Fu_g}}}
\newcommand{\phiAdg}{\varphi_{A_{\Fd_g}}}

\def\order#1{\ensuremath{{\cal O}(#1)}}
\def\reffi#1{\mbox{Fig.~\ref{#1}}}
\def\reffis#1{\mbox{Figs.~\ref{#1}}}
\def\als{\alpha_s}
\def\alt{\alpha_t}
\def\alb{\alpha_b}
\def\Ga{\Gamma}
\def\ga{\gamma}
\def\De{\Delta}
\def\de{\delta}
\def\la{\lambda}
\def\phia{\varphi_{A}}
\def\phiAt{\varphi_{\At}}
\def\phiAtb{\varphi_{A_{t,b}}}
\def\phiAb{\varphi_{\Ab}}
\def\phiAtau{\varphi_{\Atau}}
\def\phiAmu{\varphi_{\Amu}}
\def\phiAe{\varphi_{\Ae}}
\def\phimu{\varphi_{\mu}}
\def\phiMe{\varphi_{M_1}}
\def\phiMz{\varphi_{M_2}}
\def\phigl{\varphi_{\gl}}
\def\MSUSY{M_{\text{SUSY}}}
\def\MSL{M_{\tilde L}}
\def\MSE{M_{\tilde E}}
\def\MSQ{M_{\tilde Q}}
\def\MSU{M_{\tilde U}}
\def\MSD{M_{\tilde D}}
\def\amususy{\ensuremath{a_\mu^{\rm SUSY}}}
\def\gmin2{\ensuremath{(g-2)_\mu}}
\def\amu{\ensuremath{a_\mu}}
\def \met  {\mbox{${E\!\!\!\!/_T}$}}
\newcommand{\ssi}{\ensuremath{\sig_p^{\rm SI}}}
\newcommand{\ssd}{\ensuremath{\sig_p^{\rm SD}}}
\newcommand{\Och}{\Omega_\chi h^2}

\definecolor{Orange}{named}{orange}
\definecolor{Purple}{named}{purple}
\definecolor{Lightblue}{cmyk}{0.9,0.1,0.1,0.3}
\definecolor{dgelborange}{cmyk}{0.,0.3,0.5, 0.}
\definecolor{Lila}{rgb}{0.5,0.,1}
\definecolor{Darkgreen}{rgb}{0.,.7,0.2}

\newcommand{\htr}[1]{{\color{red} #1}}
\newcommand{\htb}[1]{{\color{blue} #1}}
\newcommand{\htg}[1]{{\color{Darkgreen} #1}}
\newcommand{\hto}[1]{{\color{Orange}  #1}}
\newcommand{\htp}[1]{{\color{purple}  #1}}
\newcommand{\htbl}[1]{{\color{Lightblue}#1}}
\newcommand{\htlb}[1]{{\color{Lightblue}#1}}
\newcommand{\htgo}[1]{{\color{dgelborange}#1}}
\newcommand{\htli}[1]{{\color{Lila}#1}}
\newcommand{\htgray}[1]{{\color{black!40} #1}}
\newcommand{\htrd}[1]{\htr{\st{#1}}}
\newcommand{\htbd}[1]{\htb{\st{#1}}}
\newcommand{\htgd}[1]{\htg{\st{#1}}}
\newcommand{\htod}[1]{\hto{\st{#1}}}
\newcommand{\htpd}[1]{\htp{\st{#1}}}
\newcommand{\htlbd}[1]{\htlb{\st{#1}}}
\newcommand{\htgod}[1]{\htgo{\st{#1}}}
\newcommand{\htlid}[1]{\htli{\st{#1}}}
\def\grey#1{\special{ps: .6 setgray}#1\special{ps: 0 setgray}}

